Benchmarking In-Hand Manipulation

The purpose of this benchmark is to evaluate the planning and control aspects of robotic in-hand manipulation systems. The goal is to assess the system's ability to change the pose of a hand-held object by either using the fingers, environment or a combination of both. Given an object surface mesh from the YCB data-set, we provide examples of initial and goal states (i.e.\ static object poses and fingertip locations) for various in-hand manipulation tasks. We further propose metrics that measure the error in reaching the goal state from a specific initial state, which, when aggregated across all tasks, also serves as a measure of the system's in-hand manipulation capability. We provide supporting software, task examples, and evaluation results associated with the benchmark. All the supporting material is available at https://robot-learning.cs.utah.edu/project/benchmarking_in_hand_manipulation

==> execution_constraints.tex <==
%%

==> experimental_protocol.tex <==
We provide software tools, r
\noindent \textbf{Object tracking} Marker tracking (Aruco, April), DART.

\noindent \textbf{Robot tracking} DART, hand-eye camera calibration tool.

\noindent \textbf{Environment setup} Setup DOPE to track the objects and show errors to help align to the proposed setup?


\TODO{\\Software packages:\\ Bala: DOPE, DART, Aruco tracking.\\ Silvia: Robot-camera calibration? April tracking.  }

\iffalse
\subsection{Goal generation guidelines}
We have generated initial and desired contact regions on most YCB objects, as shown in Fig.~\ref{fig:ycb_contact_regions}.
\BS{Objects:
\begin{enumerate}
    \item Banana
    \item Spatula
    \item toy-plane
    \item Plate
\end{enumerate}}

\BS{Talk about generating own set of goals}
\begin{figure}
    \centering
    %\includegraphics{pictures/task_illustration}
    \caption{Placeholder for contact regions}
    \label{fig:ycb_contact_regions}
\end{figure}

\subsection{Trials}
We do not restrict the in-hand manipulation task to be executed with a specific
robot or gripper. We encourage all kinds of different manipulation systems,
such as single-dexterous-hand systems, dual-arm-gripper systems, and systems
using external fixtures. In this way, we can evaluate the capabilities of different
manipulation strategies. Because of this, depending on the considered system, not all the tasks can be achieved because of possible mechanical limitations. For instance, a parallel gripper cannot freely move an object in-hand in all directions. These limitations can be specified when reporting the results, as they provide information on the system's in-hand manipulation capabilities as a whole, regardless of the considered in-hand manipulation strategy.

Since we want to evaluate different kinds of in-hand manipulation strategies; therefore, the prior information can assume all the knowledge that is required by the
considered planner or controller (e.g. mass, friction, object’s shape). The knowledge assumption should be specified when presenting the results.

\BS{Talk about what is definitely not allowed, such as human intervention?}
\subsection{Reporting Errors}
\subsection{Software}
\BS{Setup software for pose detection, object tracking, robot tracking}
\fi

